Enhancing the Generalization for Intent Classification and Out-of-Domain Detection in SLU

Intent classification is a major task in spoken language understanding (SLU). Since most models are built with pre-collected in-domain (IND) training utterances, their ability to detect unsupported out-of-domain (OOD) utterances has a critical effect in practical use. Recent works have shown that using extra data and labels can improve the OOD detection performance, yet it could be costly to collect such data. This paper proposes to train a model with only IND data while supporting both IND intent classification and OOD detection. Our method designs a novel domain-regularized module (DRM) to reduce the overconfident phenomenon of a vanilla classifier, achieving a better generalization in both cases. Besides, DRM can be used as a drop-in replacement for the last layer in any neural network-based intent classifier, providing a low-cost strategy for a significant improvement. The evaluation on four datasets shows that our method built on BERT and RoBERTa models achieves state-of-the-art performance against existing approaches and the strong baselines we created for the comparisons.

==> body/abstract.tex <==
\begin{abstract}
% 	Intent classification is a major task in spoken language understanding (SLU).
% 	Since most models are built with pre-collected in-domain (IND) training utterances, their ability to detect unsupported out-of-domain (OOD) utterances is critical in practice.
% 	Recent works showed that using extra data and labels can improve the OOD detection performance, yet it could be costly to collect such data.
% 	Unfortunately, existing approaches either cannot support both tasks simultaneously or heavily rely on extra information.
% 	In this paper, we propose to train a joint model only on IND training set to support both IND intent classification and OOD detection.
% 	Our method explicitly models a domain variable to learn the domain disentangled utterance representation, named \emph{DDM model}.
% 	DDM can be used as a drop-in replacement for any deep neural intent classifier.
% 	To further improve OOD detection performance, we introduce confidence and feature based OOD detection methods to combine with DDM and BERT-based models.
% 	On all existing three benchmark SLU datasets and one in-house dataset, we show that our method built on BERT and RoBERTa models achieve state-of-the-art performance against existing approaches as well as multiple BERT-based strong baselines for both intent classification and OOD detection tasks.
\end{abstract}


==> body/impact.tex <==
\section*{Impact Statement}

Our proposed method in this paper has been deployed in the domain classification SLU model for Samsung Bixby voice assistant.
In addition to SLU, our work could have a broader impact on other applications, which can be benefited from having a more robust classification system.
For example, our method can help the robot to detect objects more accurately or stop safely by correctly identifying unknown objects, classify environmental sounds or detect anomaly sounds, and so on.
Moreover, by better detecting the OOD samples that are different from the training data distribution, our method can facilitate to handle distributional shifts between training data and practical usage data.


==> body/title.tex <==
\title{Learning Domain Disentangled Representation \\
for Intent Classification and Out-of-Domain Detection in SLU}

%\author{
%	Yilin Shen, Avik Ray, Yen-Chang Hsu, Hongxia Jin \\
%	Samsung Research America, Mountain View, CA, USA \\
%	{\tt \footnotesize \{yilin.shen,hongxia.jin\}@samsung.com}
%}

